AttendLight: Universal Attention-Based Reinforcement Learning Model for Traffic Signal Control

We propose AttendLight, an end-to-end Reinforcement Learning (RL) algorithm for the problem of traffic signal control. Previous approaches for this problem have the shortcoming that they require training for each new intersection with a different structure or traffic flow distribution. AttendLight solves this issue by training a single, universal model for intersections with any number of roads, lanes, phases (possible signals), and traffic flow. To this end, we propose a deep RL model which incorporates two attention models. The first attention model is introduced to handle different numbers of roads-lanes; and the second attention model is intended for enabling decision-making with any number of phases in an intersection. As a result, our proposed model works for any intersection configuration, as long as a similar configuration is represented in the training set. Experiments were conducted with both synthetic and real-world standard benchmark data-sets. The results we show cover intersections with three or four approaching roads; one-directional/bi-directional roads with one, two, and three lanes; different number of phases; and different traffic flows. We consider two regimes: (i) single-environment training, single-deployment, and (ii) multi-environment training, multi-deployment. AttendLight outperforms both classical and other RL-based approaches on all cases in both regimes.

==> att_utils.tex <==
\pgfmathsetmacro{\WIDTH}{.8cm}
\pgfmathsetmacro{\HEIGHT}{.5cm}
\pgfmathsetmacro{\DISTANCE}{.55cm}


\tikzstyle{rect1} = [rectangle,text width=.75cm, minimum width=\WIDTH, minimum height=\HEIGHT, text centered, draw=black, fill=white!30, node distance=\DISTANCE]
% \tikzstyle{rect1} = [rectangle,text width=.4cm, minimum width=.5cm, minimum height=.6cm, text centered, draw=black, fill=white!30, node distance=1.1cm]



\pgfmathsetmacro{\PHII}{4}
\pgfmathsetmacro{\PSI}{4}
% \tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
%   1 with \arrow[semithick]{open triangle 60}},
%   double distance=1.4pt, shorten >= 5.5pt,
%   preaction = {decorate},
%   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]

% \tikzset{>=latex}
\tikzset{
  myarrow/.style = {line width=2mm, draw=blue, -triangle 60, fill=blue!40,postaction={draw, line width=4mm, shorten >=6mm, -}}
}

% \tikzset{
% fncyarrow/.style = {}
% > = stealth, % arrow head style
%         shorten > = 1pt, % don't touch arrow head to node
%         auto,
%         node distance = 3cm, % distance between nodes
%         semithick

% \tikzset{%
%   tipA/.tip={Bar[sep]Triangle[open,angle=45:4pt]},
%   tipB/.tip={Bar[sep]Square[open]}
% }

% \tikzset{
%   invisible/.style={opacity=0},
%   visible on/.style={alt={#1{}{invisible}}},
%   alt/.code args={<#1>#2#3}{%
%     \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
%   },
% }

==> box_utils.tex <==
%====================================
%emphasize vertices --> switch and emph style (e.g. thick,black)
%====================================
\makeatletter
% Standard Values for Parameters
\newcommand{\tikzcuboid@shiftx}{0}
\newcommand{\tikzcuboid@shifty}{0}
\newcommand{\tikzcuboid@dimx}{3}
\newcommand{\tikzcuboid@dimy}{3}
\newcommand{\tikzcuboid@dimz}{3}
\newcommand{\tikzcuboid@scale}{1}
\newcommand{\tikzcuboid@densityx}{1}
\newcommand{\tikzcuboid@densityy}{1}
\newcommand{\tikzcuboid@densityz}{1}
\newcommand{\tikzcuboid@rotation}{0}
\newcommand{\tikzcuboid@anglex}{0}
\newcommand{\tikzcuboid@angley}{90}
\newcommand{\tikzcuboid@anglez}{225}
\newcommand{\tikzcuboid@scalex}{1}
\newcommand{\tikzcuboid@scaley}{1}
\newcommand{\tikzcuboid@scalez}{sqrt(0.5)}
\newcommand{\tikzcuboid@linefront}{black}
\newcommand{\tikzcuboid@linetop}{black}
\newcommand{\tikzcuboid@lineright}{black}
\newcommand{\tikzcuboid@fillfront}{white}
\newcommand{\tikzcuboid@filltop}{white}
\newcommand{\tikzcuboid@fillright}{white}
\newcommand{\tikzcuboid@shaded}{N}
\newcommand{\tikzcuboid@shadecolor}{black}
\newcommand{\tikzcuboid@shadeperc}{25}
\newcommand{\tikzcuboid@emphedge}{N}
\newcommand{\tikzcuboid@emphstyle}{thick}

% Definition of Keys
\define@key{tikzcuboid}{shiftx}[\tikzcuboid@shiftx]{\renewcommand{\tikzcuboid@shiftx}{#1}}
\define@key{tikzcuboid}{shifty}[\tikzcuboid@shifty]{\renewcommand{\tikzcuboid@shifty}{#1}}
\define@key{tikzcuboid}{dimx}[\tikzcuboid@dimx]{\renewcommand{\tikzcuboid@dimx}{#1}}
\define@key{tikzcuboid}{dimy}[\tikzcuboid@dimy]{\renewcommand{\tikzcuboid@dimy}{#1}}
\define@key{tikzcuboid}{dimz}[\tikzcuboid@dimz]{\renewcommand{\tikzcuboid@dimz}{#1}}
\define@key{tikzcuboid}{scale}[\tikzcuboid@scale]{\renewcommand{\tikzcuboid@scale}{#1}}
\define@key{tikzcuboid}{densityx}[\tikzcuboid@densityx]{\renewcommand{\tikzcuboid@densityx}{#1}}
\define@key{tikzcuboid}{densityy}[\tikzcuboid@densityy]{\renewcommand{\tikzcuboid@densityy}{#1}}
\define@key{tikzcuboid}{densityz}[\tikzcuboid@densityz]{\renewcommand{\tikzcuboid@densityz}{#1}}
\define@key{tikzcuboid}{rotation}[\tikzcuboid@rotation]{\renewcommand{\tikzcuboid@rotation}{#1}}
\define@key{tikzcuboid}{anglex}[\tikzcuboid@anglex]{\renewcommand{\tikzcuboid@anglex}{#1}}
\define@key{tikzcuboid}{angley}[\tikzcuboid@angley]{\renewcommand{\tikzcuboid@angley}{#1}}
\define@key{tikzcuboid}{anglez}[\tikzcuboid@anglez]{\renewcommand{\tikzcuboid@anglez}{#1}}
\define@key{tikzcuboid}{scalex}[\tikzcuboid@scalex]{\renewcommand{\tikzcuboid@scalex}{#1}}
\define@key{tikzcuboid}{scaley}[\tikzcuboid@scaley]{\renewcommand{\tikzcuboid@scaley}{#1}}
\define@key{tikzcuboid}{scalez}[\tikzcuboid@scalez]{\renewcommand{\tikzcuboid@scalez}{#1}}
\define@key{tikzcuboid}{linefront}[\tikzcuboid@linefront]{\renewcommand{\tikzcuboid@linefront}{#1}}
\define@key{tikzcuboid}{linetop}[\tikzcuboid@linetop]{\renewcommand{\tikzcuboid@linetop}{#1}}
\define@key{tikzcuboid}{lineright}[\tikzcuboid@lineright]{\renewcommand{\tikzcuboid@lineright}{#1}}
\define@key{tikzcuboid}{fillfront}[\tikzcuboid@fillfront]{\renewcommand{\tikzcuboid@fillfront}{#1}}
\define@key{tikzcuboid}{filltop}[\tikzcuboid@filltop]{\renewcommand{\tikzcuboid@filltop}{#1}}
\define@key{tikzcuboid}{fillright}[\tikzcuboid@fillright]{\renewcommand{\tikzcuboid@fillright}{#1}}
\define@key{tikzcuboid}{shaded}[\tikzcuboid@shaded]{\renewcommand{\tikzcuboid@shaded}{#1}}
\define@key{tikzcuboid}{shadecolor}[\tikzcuboid@shadecolor]{\renewcommand{\tikzcuboid@shadecolor}{#1}}
\define@key{tikzcuboid}{shadeperc}[\tikzcuboid@shadeperc]{\renewcommand{\tikzcuboid@shadeperc}{#1}}
\define@key{tikzcuboid}{emphedge}[\tikzcuboid@emphedge]{\renewcommand{\tikzcuboid@emphedge}{#1}}
\define@key{tikzcuboid}{emphstyle}[\tikzcuboid@emphstyle]{\renewcommand{\tikzcuboid@emphstyle}{#1}}
% Commands
\newcommand{\tikzcuboid}[1]{
    \setkeys{tikzcuboid}{#1} % Process Keys passed to command
    \pgfmathsetmacro{\vectorxx}{\tikzcuboid@scalex*cos(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\vectorxy}{\tikzcuboid@scalex*sin(\tikzcuboid@anglex)}
    \pgfmathsetmacro{\vectoryx}{\tikzcuboid@scaley*cos(\tikzcuboid@angley)}
    \pgfmathsetmacro{\vectoryy}{\tikzcuboid@scaley*sin(\tikzcuboid@angley)}
    \pgfmathsetmacro{\vectorzx}{\tikzcuboid@scalez*cos(\tikzcuboid@anglez)}
    \pgfmathsetmacro{\vectorzy}{\tikzcuboid@scalez*sin(\tikzcuboid@anglez)}
    \begin{scope}[xshift=\tikzcuboid@shiftx, yshift=\tikzcuboid@shifty, scale=\tikzcuboid@scale, rotate=\tikzcuboid@rotation, x={(\vectorxx,\vectorxy)}, y={(\vectoryx,\vectoryy)}, z={(\vectorzx,\vectorzy)}]
    \pgfmathsetmacro{\steppingx}{1/\tikzcuboid@densityx}
    \pgfmathsetmacro{\steppingy}{1/\tikzcuboid@densityy}
    \pgfmathsetmacro{\steppingz}{1/\tikzcuboid@densityz}
    \newcommand{\dimx}{\tikzcuboid@dimx}
    \newcommand{\dimy}{\tikzcuboid@dimy}
    \newcommand{\dimz}{\tikzcuboid@dimz}
    \pgfmathsetmacro{\secondx}{2*\steppingx}
    \pgfmathsetmacro{\secondy}{2*\steppingy}
    \pgfmathsetmacro{\secondz}{2*\steppingz}
    
    \ifthenelse{\equal{\dimx}{1}}
    {\foreach \x in {\steppingx,...,\dimx}}
    {\foreach \x in {\steppingx,\secondx,...,\dimx}}
    {   \ifthenelse{\equal{\dimy}{1}}
        {\foreach \y in {\steppingy,...,\dimy}}
        {\foreach \y in {\steppingy,\secondy,...,\dimy}}
        {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}
            \pgfmathsetmacro{\lowy}{(\y-\steppingy)}
            \filldraw[fill=\tikzcuboid@fillfront,draw=\tikzcuboid@linefront] (\lowx,\lowy,\dimz) -- (\lowx,\y,\dimz) -- (\x,\y,\dimz) -- (\x,\lowy,\dimz) -- cycle;

        }
    }
    \ifthenelse{\equal{\dimx}{1}}
    {\foreach \x in {\steppingx,...,\dimx}}
    {\foreach \x in {\steppingx,\secondx,...,\dimx}}
    {   \ifthenelse{\equal{\dimz}{1}}
        {\foreach \z in {\steppingz,...,\dimz}}
        {\foreach \z in {\steppingz,\secondz,...,\dimz}}
        {   \pgfmathsetmacro{\lowx}{(\x-\steppingx)}
            \pgfmathsetmacro{\lowz}{(\z-\steppingz)}
            \filldraw[fill=\tikzcuboid@filltop,draw=\tikzcuboid@linetop] (\lowx,\dimy,\lowz) -- (\lowx,\dimy,\z) -- (\x,\dimy,\z) -- (\x,\dimy,\lowz) -- cycle;
        }
    }
    \ifthenelse{\equal{\dimy}{1}}
    {\foreach \y in {\steppingy,...,\dimy}}
    {\foreach \y in {\steppingy,\secondy,...,\dimy}}
    {   \ifthenelse{\equal{\dimz}{1}}
        {\foreach \z in {\steppingz,...,\dimz}}
        {\foreach \z in {\steppingz,\secondz,...,\dimz}}
        {   \pgfmathsetmacro{\lowy}{(\y-\steppingy)}
            \pgfmathsetmacro{\lowz}{(\z-\steppingz)}
            \filldraw[fill=\tikzcuboid@fillright,draw=\tikzcuboid@lineright] (\dimx,\lowy,\lowz) -- (\dimx,\lowy,\z) -- (\dimx,\y,\z) -- (\dimx,\y,\lowz) -- cycle;
        }
    }
    \ifthenelse{\equal{\tikzcuboid@emphedge}{Y}}%
        {\draw[\tikzcuboid@emphstyle](0,\dimy,0) -- (\dimx,\dimy,0) -- (\dimx,\dimy,\dimz) -- (0,\dimy,\dimz) -- cycle;%
        \draw[\tikzcuboid@emphstyle] (0,0,\dimz) -- (0,\dimy,\dimz) -- (\dimx,\dimy,\dimz) -- (\dimx,0,\dimz) -- cycle;%
        \draw[\tikzcuboid@emphstyle](\dimx,0,0) -- (\dimx,\dimy,0) -- (\dimx,\dimy,\dimz) -- (\dimx,0,\dimz) -- cycle;%
        }%
        {}
    \end{scope}
}


==> phase_utils.tex <==
\definecolor{grass}{HTML}{297301}
\definecolor{way}{HTML}{373737}

\tikzset{wbg/.style={
            rectangle,
            fill=white,
            draw,
            },
        vecArrow/.style={
            thick,
            black,
            rounded corners=.2cm,
            decoration={markings,mark=at position
            1 with {\arrow[scale=1.5,thick,black, >=stealth]{>}}},
            double distance=1.1pt, shorten >= 4.pt,
            preaction = {decorate},
            postaction = {draw,line width=1.4pt, black ,shorten >= 3.5pt}
            },
        } 
        
        
 \def\leftturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.35);
   \end{scope}
 }
  \def\straight(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 \def\rightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.35);
   \end{scope}
 }
 \def\straightleftturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (.2,0) -- (.45,.4);
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 
  \def\straightrightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.2,0) -- (.45,.4);
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 
   \def\lefttrightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.25);
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,-.25);
   \end{scope}
 }

==> tikz_utils.tex <==
\definecolor{grass}{HTML}{36EC38}
\definecolor{way}{HTML}{373737}
\definecolor{DarkCompass}{HTML}{9C9F9C}
\definecolor{LightCompass}{HTML}{BFC6BF}



\tikzset{bg/.style={
            rectangle,
            fill=grass,
            },
        road3 node/.style={% Runway 
            % sharp corners,
            way,
            line width=54pt,
            preaction={
                draw,
                way,
                line width=60pt,
                },
            preaction={
                draw,
                yellow,
                line width=55pt, % Yellow border lines.
                },
            postaction={
                draw,
                white,
                line width=20pt,
                dash pattern=on 15pt off 14pt, % Here control the road division lines
                },
            postaction={
                draw,
                way,
                line width=18pt,
                },
            },
        %STYLES
        road2 node/.style={
            rounded corners,
            way,
            line width=36pt,
            preaction={
                draw,
                way,
                line width=42pt,
                },
            preaction={
                draw,
                yellow,
                line width=37pt, % Yellow border lines.
                },
            postaction={
                draw,
                white,
                line width=1pt,
                dash pattern=on 15pt off 14pt, % Here control the road division lines
                },
            },
        road1 node/.style={
            rounded corners,
            way,
            line width=18pt,
            preaction={
                draw,
                way,
                line width=24pt,
                },
            preaction={
                draw,
                yellow,
                line width=19pt, % Yellow border lines.
                },
            },
        vecArrow/.style={
            thick,
            white,
            rounded corners=.2cm,
            decoration={markings,mark=at position
            1 with {\arrow[scale=1.5,thick,white, >=stealth]{>}}},
            double distance=1.1pt, shorten >= 4.pt,
            preaction = {decorate},
            postaction = {draw,line width=1.1pt, white ,shorten >= 4.5pt}
            },
        compass/.pic = {
            \foreach[count=\i,evaluate={\m=div(\i-1,4);\a=90*\i-90*(\m+1)}] \d in {E,N,W,S}{
              \filldraw[pic actions,rotate=\a,scale=.7+.3] (0,0) -- (45:1)--(0:3) node[transform shape,rotate=-90,above]{\fontsize{35}{40}\selectfont \d};
              \filldraw[pic actions,fill=LightCompass,rotate=\a,scale=.7+.3] (0,0) -- (-45:1)--(0:3)--cycle;
            };
            },
        } 
        
        
 \def\intersection12(#1){
 \begin{scope}[shift={(#1)}]
    \draw[fill=way, way] (-37.7pt,-37.5pt) rectangle (37.7pt,38.5pt);
 \end{scope}
 }  
 
  \def\leftturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.35);
   \end{scope}
 }
  \def\straight(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 \def\rightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.35);
   \end{scope}
 }
 \def\straightleftturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}]
      \draw[vecArrow] (0,0) -- (.2,0) -- (.45,.4);
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 
  \def\straightrightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.2,0) -- (.45,.4);
      \draw[vecArrow] (0,0) -- (0.6,0);
   \end{scope}
 }
 
   \def\lefttrightturn(#1)#2{
   \begin{scope}[shift={(#1)}, rotate={(#2)}, yscale=-1]
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,.25);
      \draw[vecArrow] (0,0) -- (.3,0) -- (.6,-.25);
   \end{scope}
 }
 
 \def\car(#1)#2{%
  \begin{scope}[shift={(#1)}, rotate={(#2)}]
    \draw[fill=red, red] (0,0) rectangle (0.4,0.8);
    \draw[->,white,>=latex,semithick] (0.2,0.4) coordinate (center) -- ++ (0,1);
    \draw[->,white,>=latex,semithick] (center) -- ++ (120:1);
    \draw[white,semithick] (center) -- ++ (90:.3) arc (90:120:.3);
    \draw[white] (center)++(105:.6) node {\small $\alpha$};
  \end{scope}
  }
